EncodingNet: A Novel Encoding-based MAC Design for Efficient Neural Network Acceleration

Deep neural networks (DNNs) have achieved great breakthroughs in many fields such as image classification and natural language processing. However, the execution of DNNs needs to conduct massive numbers of multiply-accumulate (MAC) operations on hardware and thus incurs a large power consumption. To address this challenge, we propose a novel digital MAC design based on encoding. In this new design, the multipliers are replaced by simple logic gates to represent the results with a wide bit representation. The outputs of the new multipliers are added by bit-wise weighted accumulation and the accumulation results are compatible with existing computing platforms accelerating neural networks. Since the multiplication function is replaced by a simple logic representation, the critical paths in the resulting circuits become much shorter. Correspondingly, pipelining stages and intermediate registers used to store partial sums in the MAC array can be reduced, leading to a significantly smaller area as well as better power efficiency. The proposed design has been synthesized and verified by ResNet18- Cifar10, ResNet20-Cifar100, ResNet50-ImageNet, MobileNetV2-Cifar10, MobileNetV2-Cifar100, and EfficientNetB0-ImageNet. The experimental results confirmed the reduction of circuit area by up to 48.79% and the reduction of power consumption of executing DNNs by up to 64.41%, while the accuracy of the neural networks can still be well maintained. The open source code of this work can be found on GitHub with link https://github.com/Bo-Liu-TUM/EncodingNet/.

==> binary_search.tex <==

\begin{algorithm}[htbp]
\caption{Binary search algorithm} % to determine the minimal bit-width and corresponding encoding system for multiplier output}
\footnotesize
\begin{algorithmic}[1]
\Statex \textbf{Input:} $BW_{min}=16, BW_{max}=128$, $RMSE_{tar.}$,
%$\textbf{\textit{v}}$, 
%$In1$, $In2$, 
$M=1e4$  // total sampling times
\Statex \textbf{Output:} $BW_{best}$% $RMSE_{best}$, $\textbf{\textit{D}}_{best}$, 

\While {$(BW_{max}-BW_{min})>1$}
    \State $BW_{mid} = \left \lceil (BW_{max}+BW_{min})/2  \right \rceil  $
    %\State $RMSE_{list}$, $D_{list}$, $s_{list}$ = [], [], []
    \For {i $in$ range($M$)}
    \State $RMSE$=eval.($BW_{mid}$)
        %\State $\textbf{\textit{D}}$ = \Call{sampling}{$logicLib, In1, In2, N$}
        %\For {i $in$ range($N$, $BW_{mid}$, -1)}
            %\State $\textbf{\textit{s}}^* = \mathop{\arg\min}\limits_{\textbf{\textit{s}}} \Vert \textbf{\textit{D}} \textbf{\textit{s}} - \textbf{\textit{v}}  \Vert_2$  // least square method
            %\State delete the column in $\textbf{\textit{D}}$ w.r.t min(abs($\textbf{\textit{s}}^*$))
            \State $RMSE_{list}$.append($RMSE$),
        % \EndFor
       % \State $e = \textbf{\textit{D}} \textbf{\textit{s}}^* - \textbf{\textit{v}}$, $RMSE=\Vert e/e.numel()\Vert_2$
       %\State $D_{list}$.append($\textbf{\textit{D}}$), $s_{list}$.append($\textbf{\textit{s}}^*$)
   \EndFor
    \State $RMSE_{min}$ = min($RMSE_{list}$)
   % \State $\textbf{\textit{D}}^*$ = the $\textbf{\textit{D}}$ in $D_{list}$ w.r.t $RMSE_{min}$
%    \State $\textbf{\textit{s}}^*$ = the $\textbf{\textit{s}}^*$ in $s_{list}$ w.r.t $RMSE_{min}$
    \If{$RMSE_{min} <= RMSE_{target}$}
        \State $BW_{max} = BW_{mid}$
        \State $BW_{best}$ = $BW_{mid}$
        \State $RMSE_{best}$ = $RMSE_{min}$
        %\State $\textbf{\textit{D}}_{best}$, $\textbf{\textit{s}}_{best}$ = $\textbf{\textit{D}}^*$, $\textbf{\textit{s}}^*$
    \Else
        \State $BW_{min} = BW_{mid}$
    \EndIf
\EndWhile

\end{algorithmic}
\label{Alg:BinarySearch}
\end{algorithm}

==> latexmkrc <==
@default_files = ("bare_jrnl_new_sample4.tex");

$bibtex_use = 2;
$pdf_mode = 1;
$pdflatex='pdflatex -synctex=1 %O %S';

add_cus_dep('vsz', 'pdf', 0, 'veusz_pdf' );
sub veusz_pdf {
system( "/Applications/Veusz.app/Contents/MacOS/veusz.exe --export=\"$_[0].svg\" --export-option=svgtextastext=True \"$_[0].vsz\"" );
return system( "inkscape -D --export-type=pdf --export-filename=\"$_[0].pdf\" \"$_[0].svg\"" ); 
}

add_cus_dep('svg', 'pdf', 0, 'inkscape_pdf' );
sub inkscape_pdf {
return system( "inkscape -D --export-type=pdf --export-filename=\"$_[0].pdf\" \"$_[0].svg\"" ); 
}


==> replies1.tex <==
\newcommand{\reviewb}{\setcounter{page}{0}\pagenumbering{roman}\thispagestyle{empty}}
\newcommand{\reviewe}{\clearpage\setcounter{page}{0}\pagenumbering{arabic}}
%\fontsize{11}{12}\selectfont
\newcommand{\spb}{\clearpage\begin{table*}\begin{center}\begin{minipage}[t][25cm][t]{14.8cm}\normalsize}
\newcommand{\spe}{\end{minipage}\end{center}\end{table*}}

\reviewb

\spb

Dear Editors, dear Reviewers,\\

Enclosed please find the revised version of the paper ``EncodingNet: A Novel Encoding-based MAC Design for Efficient Neural Network Acceleration". 
This paper was reviewed for IEEE TCASAI and a major revision was required, 
which we have done in this version according to the comments and suggestions from the reviewers.\\

We thank the editors and the reviewers sincerely for giving us the constructive
comments and suggestions to improve this manuscript.\\

The textual changes in this manuscript are highlighted using blue color. A
detailed discussion 
%on the changes and the comments in the reviews 
is given as
follows, where the comments from the reviewers are printed in italics.\\

\vspace{20pt}

\textbf{Reviewer: 1} \\

\textit{Comments to the Author}\\
\vskip -5pt

\textit{This paper presents a novel encoding method that changes the position weight of the output bit sequence of the multiplier, making it different from the common binary complement. This paper also gives the design of MAC array and algorithm evaluation, which constitutes a relatively complete system. However, there are some major concerns that need to be answered and supplemented by the author.}\\

Thanks for the comments. We address your concerns as follows.\\

\vskip 10pt

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textit{1. The search process for approximate multiplier in this paper seems to be time consuming. The three-layer loop in Algorithm 1 causes the genetic algorithm to be run 81 times, and the process of running the genetic algorithm is complicated each time. In this case, it is better for the author to provide details such as the running time of the search process, the running platform, etc., so that the reader can better understand the advantages and disadvantages of the proposed method.}\\

\vskip 5pt

Thanks for the comments. In fact, the three-layer loop in Algorithm (\ref{Alg:grid_search}) causes the genetic algorithm to run 27 times.
%, instead of 81 times. And 
%The runtime for various configurations is different. If we run 
For evaluation of the runtime, the details of runtime of the genetic algorithm with 2500 generations on a 4-core CPU (Xeon E-2124G 3.40 GHz 32 GB RAM) with one GPU card (Quadro RTX 6000 24 GB) are shown in Table \ref{tab:running time}. 
%But these search tasks are parallel, so we can run them on different severs simultaneously.
In implementing this algorithm, the searching process can be executed on multiple servers simultaneously. In the experiments
we actually ran them on 15 servers, and the total time of running Algorithm (\ref{Alg:grid_search}) was around 20.5 hours.  After the encoding-based multiplier is searched, it can be used in all the following experiments. Since this search process needs to be executed only once and offline, the runtime is still reasonable in the proposed context. This information has been added and highlighted in Section~\ref{Setup for Hardware Synthesis}.
\\

{\footnotesize

\centering

\caption{Runtime on a 4-core CPU (Xeon E-2124G 3.40 GHz 32 GB RAM) with one GPU card (Quadro RTX 6000 24 GB)}.
\begin{tabular}{cccccccccccccc}
\toprule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}logic \\level\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}logic \\depth\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}output \\nodes\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} runtime \\(h)\end{tabular}}
& 
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}logic \\level\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}logic \\depth\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}output \\nodes\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} runtime \\(h)\end{tabular}}
& 
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}logic \\level\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}logic \\depth\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}output \\nodes\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} runtime \\(h)\end{tabular}}
\\ \midrule
1 & 64  & 64 & 4.39 &  & 1 & 64  & 128 & 7.75  &  & 1 & 64  & 256 & 14.18 \\
2 & 64  & 64 & 4.53 &  & 2 & 64  & 128 & 8.08  &  & 2 & 64  & 256 & 14.99 \\
3 & 64  & 64 & 4.67 &  & 3 & 64  & 128 & 8.27  &  & 3 & 64  & 256 & 15.65 \\
1 & 128 & 64 & 4.50 &  & 1 & 128 & 128 & 8.03  &  & 1 & 128 & 256 & 14.27 \\
2 & 128 & 64 & 4.74 &  & 2 & 128 & 128 & 8.34  &  & 2 & 128 & 256 & 15.51 \\
3 & 128 & 64 & 5.21 &  & 3 & 128 & 128 & 9.17  &  & 3 & 128 & 256 & 17.37 \\
1 & 256 & 64 & 4.63 &  & 1 & 256 & 128 & 8.24  &  & 1 & 256 & 256 & 15.17 \\
2 & 256 & 64 & 5.33 &  & 2 & 256 & 128 & 9.22  &  & 2 & 256 & 256 & 17.10 \\
3 & 256 & 64 & 6.40 &  & 3 & 256 & 128 & 11.10 &  & 3 & 256 & 256 & 20.28 \\
\bottomrule
\end{tabular}
\label{tab:running time}

}

\vskip 20pt

\spe\spb

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textit{2. Genetic algorithm itself lacks rigorous theoretical analysis. Initial conditions and random operation affect the possibility of finding useful circuits. Therefore, the authors should analyze the success rate of the circuit search process, and the average cost reduction (since the circuit cannot be optimal during each search).}\\

Thanks for your comments. 
%We indeed overlooked the analysis of the applied CGP algorithm. For simplicity, we let 
In this paper, we determined the parameters based on the convergence of the genetic algorithm. We tried many parameter combinations and allowed the algorithm to evolve for 100 generations. The parameter combination with the fastest convergence was used as the configuration for our subsequent search. Now we try to analyze the GCP algorithm, and explain our parameters configuration.\\

\textbf{Analysis setup and notations:}\\
For analyzing the GCP algorithm, we use the example with
logic level $c$ = 2, logic depth $r$ = 64, output nodes $m$ = 256, output bits $M$ = 64, maximal relative error threshold $\varepsilon_{th}$ = 0.1\%, and $n_{\text{generations}}$=2500. $\varepsilon$ denotes the maximal relative error of the searched multiplier after 2500 generations. 
$n_{\text{parents}}$, $n_{\text{offsprings}}$, and $n_{\text{champions}}$ denote the number of parents, offsprings and champions in CGP algorithm.\\


\textbf{Initial conditions:}\\
Population parameters, such as $n_{\text{parents}}$, $n_{\text{offsprings}}$, and $n_{\text{champions}}$ determine the size of population we keep from the last generation, and the size of new individuals we create in the next generation. Large size of population will explore more search space, but also increase the search time. And the impotance of each population parameter is different. For example, in Table \ref{tab:Initial conditions}, we can see that the number of offsprings $n_{\text{offsprings}}$ plays a crucial role in reducing the maximum relative error $\varepsilon$. The larger the $n_{\text{offsprings}}$ is, the lower $\varepsilon$ will be achieved. So we set $n_{\text{offsprings}}$ to a large value, i.e. 50. While for the number of champions $n_{\text{champions}}$ from 1 to 5, the CGP algorithm reaches a similar $\varepsilon$, which means we can set $n_{\text{champions}}$ to a relatively small number to save search time, i.e. 2.  For small and large number of parents $n_{\text{parents}}$, we can both reach smaller $\varepsilon$. So, larger $n_{\text{parents}}$ might be helpful to improve the success rate, but it also increase the runtime. After the trade-off between the success rate and the running time, we finally set $n_{\text{parents}}$=10. \\


{

\centering
\footnotesize
\caption{Initial conditions analysis.}
\begin{tabular}{ccccccccc}
\toprule
  % \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}index\end{tabular}}
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}$n_{\text{parents}}$\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}$n_{\text{offsprings}}$\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}$n_{\text{champions}}$\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Mutation \\rate\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}MUL \\$\varepsilon$\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}MUL \\area (um$^2$)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Meet $\varepsilon_{th}$ \\($\varepsilon \le \varepsilon_{th}$)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Area (mm$^2$)\\64$\times$64\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Power (W)\\64$\times$64\end{tabular}}
\\ \midrule
10 & 10 & 2 & dynamic & 0.122\% & 19.01 & No  & 0.581 & 2.097 \\
10 & 20 & 2 & dynamic & 0.134\% & 17.24 & No  & 0.578 & 2.093 \\
10 & 30 & 2 & dynamic & 0.104\% & 20.12 & No  & 0.665 & 2.841 \\
10 & 40 & 2 & dynamic & 0.098\% & 14.75 & Yes & 0.627 & 2.476 \\
10 & 50 & 2 & dynamic & 0.098\% & 14.02 & Yes & 0.580 & 2.168 \\\midrule
10 & 50 & 1 & dynamic & 0.116\% & 21.56 & No  & 0.655 & 3.054 \\
10 & 50 & 2 & dynamic & 0.098\% & 14.02 & Yes & 0.580 & 2.168 \\
10 & 50 & 3 & dynamic & 0.104\% & 19.86 & No  & 0.591 & 2.463 \\
10 & 50 & 4 & dynamic & 0.098\% & 15.73 & Yes & 0.680 & 2.966 \\
10 & 50 & 5 & dynamic & 0.110\% & 18.81 & No  & 0.587 & 2.234 \\\midrule
10 & 50 & 2 & dynamic & 0.098\% & 14.02 & Yes & 0.580 & 2.168 \\
20 & 50 & 2 & dynamic & 0.134\% & 16.91 & No  & 0.585 & 2.303 \\
30 & 50 & 2 & dynamic & 0.153\% & 16.38 & No  & 0.579 & 2.145 \\
40 & 50 & 2 & dynamic & 0.098\% & 15.60 & Yes & 0.582 & 2.234 \\
50 & 50 & 2 & dynamic & 0.104\% & 18.09 & No  & 0.611 & 2.624 \\
\bottomrule
\end{tabular}
\label{tab:Initial conditions}

}

\vskip 20pt

\textbf{Random operations:}\\
The mutation rate has a significant impact on the stability of the evolutionary algorithm. Large mutation rate hinder the algorithm from converging. Small mutation rate enlarge the number of iterations. There are two strategies for setting the mutation rate. The first strategy is to set it as a fixed value, keeping it constant throughout the evolution process. The second strategy is to dynamically adjust the mutation rate based on a specific parameter. In our algorithm, we 
dynamically adjuste the mutation rate based on the maximum relative error $\varepsilon$ of champions. If champions reach a large $\varepsilon$, we make mutation rate bigger to explore more search space. If champions reach a small $\varepsilon$, we lower mutation rate to help the CGP algorithm to converge. In Table \ref{tab:Random operations}, dynamical strategy achieves better $\varepsilon$, power, and area, compared with strategies with fixed mutation rates.\\

\spe\spb

{

\centering
\footnotesize
\caption{Random operations analysis.}
\begin{tabular}{ccccccccc}
\toprule
  % \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}index\end{tabular}}
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}$n_{\text{parents}}$\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}$n_{\text{offsprings}}$\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}$n_{\text{champions}}$\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Mutation \\rate\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}MUL \\$\varepsilon$\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}MUL \\area (um$^2$)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Meet $\varepsilon_{th}$ \\($\varepsilon \le \varepsilon_{th}$)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Area (mm$^2$)\\64$\times$64\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Power (W)\\64$\times$64\end{tabular}}
\\ \midrule
10 & 50 & 2 & dynamic & 0.098\% & 14.02 & Yes & 0.580 & 2.168 \\
10 & 50 & 2 & 1\%     & 0.098\% & 16.25 & Yes & 0.589 & 2.433 \\
10 & 50 & 2 & 2.5\%   & 0.171\% & 19.07 & No  & 0.689 & 3.128 \\
10 & 50 & 2 &   5\%   & 0.336\% & 18.68 & No  & 0.662 & 3.017 \\
10 & 50 & 2 & 10\%    & 2.069\% & 21.56 & No  & 0.590 & 2.330 \\
10 & 50 & 2 & 15\%    & 3.326\% & 20.51 & No  & 0.582 & 2.128 \\
10 & 50 & 2 & 20\%    & 4.193\% & 20.12 & No  & 0.585 & 2.337 \\

\bottomrule
\end{tabular}
\label{tab:Random operations}

}

\vskip 20pt

\textbf{Success rate:}\\
The CGP search algorithm has two stages. In the first stage, the maximum relative error $\varepsilon$ will be reduced towards $\varepsilon_{th}$. If $\varepsilon$ $\le$ $\varepsilon_{th}$, the algorithm goes to the second stage. In the second stage, the area of the multiplier will be reduce as small as possible. 
So, the success rate of the CGP search algorithm can be defined as the probability that the $\varepsilon_{th}$ can be met. 
To analyze the success rate, we repeatedly run the CGP search algorithm 10 times with the same parameters configuration, as shown in Table \ref{tab:Success rate}. 
The CGP algorithm successfully met the threshold $\varepsilon_{th}$ 3 times out of 10, so the success rate is around 30\%.
The success rate is indeed somewhat low, but the advantage is that it allows for extensive parallel search, saving search time.\\


\textbf{Average cost reduction:}\\
The average cost reduction can be also obtained from Table \ref{tab:Success rate}. Compared with the area and power of 64$\times$64 systolic array, the average cost reduction in area and power is 21.87\% and 36.12\%, respectively. The average cost reduction is close to the best reduction we report in our final results, indicating that our algorithm demonstrates a good stability and convergence.

% The results of the algorithm are reported in  Table~\ref{tab:Success rate} -- Table~\ref{tab:Random operations}, in which \textcolor{red}{different numbers of parents, offsprings, and champions are used}.
% Area and power of 64$\times$64 MAC arrays 
% % based on the searched multipliers 
% are shown in the last two columns of these tables. 

% We analyse the CGP algorithm in three aspects:
% \begin{itemize}
%   \item \textit{Success rate}: We repeatedly ran the CGP search algorithm 10 times with $n_{\text{parents}}$=10, $n_{\text{offsprings}}$=50, $n_{\text{champions}}$=2, and dynamically adjusted mutation rate strategy to examine the success rate. As shown in Table \ref{tab:Success rate}, the CGP algorithm successfully met the threshold $\varepsilon_{th}$ 3 times out of 10, \textcolor{red}{so that the success rate is around 30\%. Compared with the area and power of 64$\times$64 systolic array, the average cost reduction in area and power is 21.87\% and 36.12\%, respectively. }
%   % \item \textit{Initial conditions}: We set $n_{\text{parents}}$, $n_{\text{offsprings}}$, and $n_{\text{champions}}$ to other values to examine the search results, as shown in Table \ref{tab:Initial conditions}. Larger $n_{\text{offsprings}}$ contributes more to decrease  $\varepsilon$. \textcolor{red}{While the $n_{\text{champions}}$ from 1 to 5 reaches similar $\varepsilon$. Larger $n_{\text{parents}}$ might improve the success rate, but it also increase the runtime.} So, we finally set $n_{\text{parents}}$=10, $n_{\text{offsprings}}$=50, and $n_{\text{champions}}$=2 after the trade-off between the success rate and the running time. 
%   \item \textit{Random operations}: We compare dynamically adjusted mutation rate strategy and fixed mutation rate strategy, as shown in Table \ref{tab:Random operations}. Compared with fixed mutation rates, dynamically adjusted strategy achieves better $\varepsilon$, power, and area simultaneously. 
% \end{itemize}

{

\centering
\footnotesize
\caption{Success rate analysis.}
\begin{tabular}{cccccccccc}
\toprule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}index\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}$n_{\text{parents}}$\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}$n_{\text{offsprings}}$\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}$n_{\text{champions}}$\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Mutation \\rate\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}MUL \\$\varepsilon$\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}MUL \\area (um$^2$)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Meet $\varepsilon_{th}$ \\($\varepsilon \le \varepsilon_{th}$)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Area (mm$^2$)\\64$\times$64\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Power (W)\\64$\times$64\end{tabular}}
\\ \midrule
1  & 10 & 50 & 2 & dynamic & 0.128\% & 18.61 & No  & 0.582 & 2.323 \\
2  & 10 & 50 & 2 & dynamic & 0.104\% & 18.87 & No  & 0.583 & 2.398 \\
3  & 10 & 50 & 2 & dynamic & 0.098\% & 14.02 & Yes & 0.580 & 2.168 \\
4  & 10 & 50 & 2 & dynamic & 0.128\% & 17.89 & No  & 0.587 & 2.466 \\
5  & 10 & 50 & 2 & dynamic & 0.098\% & 16.06 & Yes & 0.584 & 2.340 \\
6  & 10 & 50 & 2 & dynamic & 0.122\% & 19.46 & No  & 0.588 & 2.306 \\
7  & 10 & 50 & 2 & dynamic & 0.122\% & 18.28 & No  & 0.609 & 2.556 \\
8  & 10 & 50 & 2 & dynamic & 0.128\% & 19.86 & No  & 0.584 & 2.418 \\
9  & 10 & 50 & 2 & dynamic & 0.098\% & 16.19 & Yes & 0.603 & 2.610 \\
10 & 10 & 50 & 2 & dynamic & 0.116\% & 19.20 & No  & 0.636 & 2.820 \\

\bottomrule
\end{tabular}
\label{tab:Success rate}

}

\vskip 30pt


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textit{3. In Table II, the authors demonstrate the superiority of the proposed MAC array only by comparing it with the traditional exact systolic array. However, what the reader would prefer to see, is a comparison with systolic array which uses approximate multipliers and an approximate adders.}\\

\vskip 5pt

Thanks for your comments. We conducted the  comparison between the proposed MAC array and systolic arrays using approximate multipliers and approximate adders and show the results below. We selected ``mul8s\_1L2H'' from \ref{ref:EvoApprox8b} as the approximate multiplier, and the approximate adder in \ref{ref:ACA-CSU}--\ref{ref:ACA-CSU-github} for this comparison. Approximate adders from \ref{ref:EvoApprox8b} are not used, because the maximum input bit-width in \textcolor{red}{\ref{ref:EvoApprox8b}} is only 16, which is not sufficient to maintain the accuracy. We used the selected approximate multiplier and adder to build a 64$\times$64 systolic array and evaluated the area and power consumption. We compiled the C codes of the approximate multiplier and adder, and then embed them to Pytorch to fine-tune the neural networks and test the accuracy. The results are shown in Table \ref{tab:systolic-approx-approx}. 
%Let [E/A] represent the configuration of the exact multiplier and approximate adder in systolic array. Compared with [E/E], [E/A] and [A/E] configurations, 
According to this comparison, the proposed design achieves better area, power and accuracy generally. Compared with the systolic array with approximate multipliers and adders, the area and power of the proposed design are slightly higher, but the accuracy is much better. This comparison has been added in Section~\ref{Accuracy and Hardware Comparison with Approximate Systolic Arrays}.


\spe\spb

{
\centering
\footnotesize
\caption{Comparison between the proposed design and systolic arrays based on approximate and accurate multipliers and accumulators.}
\begin{tabular}{ccccccccc}
\toprule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Architecture\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Multiplier\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Adder\end{tabular}}
% & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Config\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Area (mm$^2$)\\64$\times$64\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Power (W)\\64$\times$64\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet18 \\(Cifar-10)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet20 \\(Cifar-100)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet50 \\(ImageNet)\end{tabular}}
\\ \midrule
systolic & exact  & exact  & 0.76 & 3.82 & 93.01\% & 68.40\% &  75.64\% \\
systolic & exact  & approx & 0.58 & 2.61 & 91.77\% & 65.55\% &  71.54\% \\
systolic & approx & exact  & 0.68 & 2.59 & 92.74\% & 67.53\% &  74.94\% \\
systolic & approx & approx & 0.54 & 2.02 & 90.34\% & 63.23\% &  68.37\% \\
proposed & ours   & exact  & 0.58 & 2.17 & 93.14\% & 68.32\% &  75.46\% \\
\bottomrule
\end{tabular}
\label{tab:systolic-approx-approx}

}

\vskip 10pt



{

\small

\begin{enumerate}[label={[}\arabic{*}{]}]
    \item\label{ref:EvoApprox8b} V. Mrazek, et al., ``EvoApprox8b:  Library of Approximate Adders and Multipliers for Circuit Design and Benchmarking of Approximation Methods," in \textit{Design, Automation \& Test in Europe Conference \& Exhibition (DATE)}, 2017.
    \item\label{ref:ACA-CSU} A. Kanani, et al., ``ACA-CSU: A Carry Selection Based Accuracy Configurable Approximate Adder Design," in \textit{IEEE Computer Society Annual Symposium on VLSI (ISVLSI)}, 2020.
    \item\label{ref:ACA-CSU-github} ``ACA-CSU," \url{https://github.com/AlishKanani/ACA-CSU_Approximate-Adders/tree/main}.
\end{enumerate}


% [1] P. Balasubramanian, et al., ``An Approximate Adder With a Near-Normal Error Distribution: Design, Error Analysis and Practical Application," in \textit{IEEE Access}, vol. 9, pp. 4518-4530, 2021.
% Another approximate adder is from \url{https://github.com/OkkarMin/approximator-tool}.

}

\vskip 25pt

% \spe\spb

\textit{4. A detailed breakdown of the MAC array should be given. The reduction in array overhead may mainly come from bit-wise ACC and weighted summation of the ACC results. If the accumulation of partial products in existing exact multiplier or approximate multiplier is merged with the accumulation of multiplication results, can the overhead be reduced as well?}\\

Thanks for the comments. For this comparison, we compared exact, approximate  (``mul8s\_1L2H'' from  \ref{ref:EvoApprox8b}), and proposed multipliers combined with the proposed bit-wise accumulation adders. The results are shown in 
%We indeed overlook the comparison between the systolic array and the proposed MAC arrays using exact or approximate multipliers.
%We build 64$\times$64 MAC array with our searched multiplier, exact multiplier and approximate multiplier (``mul8s\_1L2H'' from \ref{ref:EvoApprox8b}), respectively. 
%The area and timing are evaluated and compared with 64$\times$64 systolic array, as 
 Table \ref{tab:prop-approx-approx}. According to this comparison, these designs have similar area overhead, but the version with exact and approximate multiplers did not meet the timing requirement as whon in the last row in Table \ref{tab:prop-approx-approx}, because these multipliers are much more complicated than the proposed multipliers. this comparison has been added in Section \ref{Hardware Comparison with Bit-Wise Accumulation of Exact and Approximate Multipliers}.

%Compared with the systolic array with exact multipliers and adders, the proposed MAC arrays with exact multipliers and approximate multipliers can indeed achieve reduced overhead, but the timing is violated because of the long critical path in these multipliers.\\

\vskip 5pt

{

\centering
\footnotesize
%\caption{Comparison between systolic array and the proposed arrays. The proposed arrays are based on multipliers of their exact, approximate, and our searched versions.}
\caption{Comparison of exact, approximate  (``mul8s\_1L2H'' from  \ref{ref:EvoApprox8b}), and proposed multipliers combined with the proposed bit-wise accumulation adders. }

\begin{tabular}{ccccccc}
\toprule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Architecture\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Multiplier\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Adder\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Area (mm$^2$)\\64$\times$64\end{tabular}}
% & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Power (W)\\64$\times$64\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Timing\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Slack (ps)\end{tabular}}
\\ \midrule

proposed & ours   & exact & 0.58 & MET      & 5.96   \\
proposed & exact  & exact & 0.60 & VIOLATED & -25.59 \\
proposed & approx & exact & 0.59 & VIOLATED & -5.64  \\
\bottomrule
\end{tabular}
\label{tab:prop-approx-approx}

}

\vskip 30pt

% \spe\spb

\textit{5. In paragraph 1 of Section IV-A, the authors say that the clock frequency is 5GHz (0.2ns), which is quite amazing. Since in Fig. 5, the circuit between Bit-wise ACC registers to output registers, contains large bit-width multipliers and an adder tree. In this case, making the critical path smaller than 0.2ns is difficult to achieve, even with the 15nm process.}\\

\vskip 5pt

This is a very nice observation.
Indeed, in Fig. 5, the circuit between bit-wise ACC registers and output registers, contains large bit-width multipliers and an adder tree. 
It seems that the critical path smaller than 0.2ns is difficult to achieve. 
%But actually,
%the ``large bit-width multipliers'' and an ``adder tree'' are not ``full'' or ``original''. They are actually logically simplified.
However, these mutlipliers and adders are not full circuits, because the coeffieincets (position weigths) to them are fixed and the circuits can be significantly reduced.
%Because the position weights in Fig. 5 are all fixed and unchanged after CGP searching. These fixed position weights are used to simplify the logic of the ``large bit-width multipliers'' and the ``adder tree''.
As an example, please find the Verilog code on the online simulation link ``\url{http://hdlbits.01xz.net/wiki/Iverilog?load=0WLucJ}'', in which a column of 2$\times$2 MAC array is implemented. In line 122-185 of this Verilog code, position weights are all defined as ``localparam'', and most of them are power of two. These values  make the multipliers and the adder tree much simpler. The synthesis tool (Design Compiler) can automatically utilize these position weights to shorten the critical paths of the circuits  to satisfy the target clock period 0.2ns.\\


\vskip 20pt

\spe\spb

\textit{6. The experimental results should be better structured. It is best to have subsections and have logical relationships between them.}\\

\vskip 5pt

Thanks for the suggestion. We have split Section \ref{sec:results} into several subsections.\\

\vskip 20pt

\textit{7. The code for this paper is strongly recommended to be open source. Because the complicated search process and the large amount of evaluation data given in the article are difficult to reproduce by readers.}\\

\vskip 5pt

Thanks for your suggestion. %The complicated search process is indeed difficult to reproduce by readers. The code is 
The open source code can be found on GitHub with link ``\url{https://github.com/Bo-Liu-TUM/EncodingNet/}''. There are 4 main Python files, where ``Code\_1\_CGP\_search.py'' is used to apply CGP search process,  ``Code\_2\_finetune\_cifar10.py'', ``Code\_3\_finetune\_cifar100.py'', and ``Code\_4\_finetune\_imagenet.py'' are used to fine-tune neural networks. These are the most important files for this paper. Remaining files will be structured and updated to the GitHub repository later. The GitHub link has also been added into the end of Section~\ref{sec:ex_setup}.\\

\vskip 20pt

\textit{8. Related works are suggested to be added. Although I think the encoding method proposed by the authors is interesting, it still has similarities with many existing works, which needs detailed comparison and analysis.}\\

\vskip 5pt

Thanks for your suggestions. Related work is reviewed as follows and added to the end of Section~\ref{sec:Motivation}. Related work majorly focuses on exploring new data representations, optimization of multipliers and MAC units, and approximate computing applied to DNNs to reduce area overhead and power consumption.  \\ 


On novel data representations, in \ref{ref:D-log-2016}, weights and activations are represented with a power of 2 by using binary logarithmic quantization. Multiplication operations are replaced by addition of exponents and bit-shifting, eliminating the need for digital multipliers and enhancing computational efficiency. However, the logarithmic number system is less efficient to represent the distribution of weights and activations, which confines the accuracy in lower bit-width data representation.
Residue number system (RNS) has also been explored to optimize the hardware implementation of convolutional layers \ref{ref:M-RNS-2020}. Multiplications and accumulations in traditional 2’s complement are replaced with the counterparts in RNS without carry propagation, which speeds up operations and improves the computational efficiency. But the residue number system suffers from a large cost of modular operations and data conversion into binary number system. 
Fibonacci encoding technique has been used to encode weights of neural networks \ref{ref:Fibonacci}, while the activations and products are still in 2's complement. 
By using the Fibonacci encoding technique, some full adders in the multipliers can be replaced with OR gates, leading to a reduced area, power and delay. 
However, the Fibonacci encoding technique requires special handling of weights, and restricts the range of representable values (especially, it cannot encode negative values), potentially affecting model expressiveness.\\

On the optimization of exact multipliers, 
multi-bit recoding is used to optimize multiplication by grouping multiple bits of the multiplier and re-encoding them to reduce the number of partial products, such as the Booth multipier and its variants \ref{ref:Booth}.
To compress the partial product towards less bits representation or less compression layers, schemes such as Wallace tree \ref{ref:Wallace} and Dadda tree \ref{ref:Dadda} are proposed. 
Overlapped multiple-bit scanning multiplication is an optimized multiplication method where multiple bits of the multiplier are processed with overlapping groups to reduce operations and improve speed \ref{ref:OMBSSM}. 
These design schemes are widely applied, but all of them rely on the 2's complement format and do not change the encoding of the multiplication output. 
Further optimization of MAC units include \ref{ref:IMAC-2024} and \ref{ref:Ponraj-2023}, where adders are integrated into multipliers.\\

\spe\spb

On approximate computing, approximate multipliers and adders have been explored in DNN accelerators to reduce the power consumption while maintaining the accuracy \ref{ref:G-Thermal-2022}.  
AutoApprox identifies which layers in a neural network are error-tolerant and implements them with approximate MAC units, while sensitive layers are implemented  with exact MAC units to maintain overall accuracy \ref{ref:P-Learning-2022}. 
ApproxNNs use approximate multipliers to reduce hardware area and energy consumption, and retrain large-scale neural networks to maintain the accuracy %because of the propagation of errors across layers 
with a controlled error \ref{ref:T-Toward-2024}. 
Table \ref{tab:sota-designs-compare} compares the proposed approach with these state-of-the-art designs, focusing on widely used datasets and networks.\\



{

\centering
\footnotesize
\caption{Comparison with state-of-the-art designs}
\begin{tabular}{cccccccc}
\toprule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Work\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Multiplier \\Type\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Multiplier \\Output \\Format\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Multiplier \\Output \\Bit-Width\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Dataset\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Model\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Acc\textsubscript{A} (\%)\textsuperscript{a}\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Acc\textsubscript{loss} (\%)\textsuperscript{c}\end{tabular}}
\\ \midrule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}DAC'21\\\ref{ref:Fibonacci}\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Approx \\8b$\times$8b\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}2's comp.\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}16b\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Cifar100\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet18\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}73.54\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}-1.74\end{tabular}}
\\ \midrule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}DATE'22\\\ref{ref:G-Thermal-2022}\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Approx \\8b$\times$8b\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}2's comp.\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}16b\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ImageNet\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet50\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}72.5\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}-\end{tabular}}
\\ \midrule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}TC'22\\\ref{ref:P-Learning-2022}\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Approx \\8b$\times$8b\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}2's comp.\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}16b\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Cifar100 \\ImageNet\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}MobileNetV2 \\ResNet18\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}-\\-\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}-2.4\\-1.3\end{tabular}}
\\ \midrule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}VLSI'24\\\ref{ref:T-Toward-2024}\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Approx \\8b$\times$6b\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}2's comp.\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}16b\textsuperscript{b}\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Cifar100\\Cifar100\\ImageNet\\ImageNet\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet18\\MobileNetV2\\ResNet18\\ResNet50\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}76.11\\67.76\\68.28\\75.0 \end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}-0.27\\-1.36\\-1.48\\-1.13\end{tabular}}
\\ \midrule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ours\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Approx \\8b$\times$8b\textsuperscript{b}\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}searched \\encoding\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}64b\textsuperscript{b}\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
Cifar10\\
Cifar100\\
ImageNet\\
Cifar10\\
Cifar100\\
ImageNet
\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
ResNet18\\
ResNet20\\
ResNet50\\
MobileNetV2\\
MobileNetV2\\
EfficientNet-B0
\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
93.14\\
68.32\\
75.46\\
93.74\\
71.23\\
68.77
\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
+0.07\\
-0.5\\
-1.59\\
-0.17\\
+0.06\\
-8.92
\end{tabular}}
\\
\bottomrule

\multicolumn{8}{l}{\begin{tabular}[l]{@{}l@{}}
\textsuperscript{a} Top-1 accuracy when using approximate multiplier \\
\textsuperscript{b} 8b means 8-bit, 6b means 6-bit, 16b means 16-bit, and 64b means 64-bit \\
\textsuperscript{c} Top-1 accuracy loss compared with the 32-bit floating-point model
\end{tabular}}\\

\end{tabular}
\label{tab:sota-designs-compare}

}

\vskip 10pt
%As to the design of approximate multipliers and adders, there are many explorations. 
%LSB (Least Significant Bit) and MSB (Most Significant Bit) are usually processed in a different way to reduce the complexity and maintain the accuracy \ref{ref:V-IMPACT-2011}.
%Bit-width of operands can be dynamically adaptated to save the power and keep the performance \ref{ref:J-Approximate-2013}. 
%Carry-skip is predicted by LSBs to reduce the delay, and k-bit segmentation is processed by sub-adders to reduce the complexity \ref{ref:Y-Energy-2014}. 
%CGP algorithm is explored to search Pareto front approximate multipliers and adders \ref{ref:EvoApprox8b-}.  
%These approximate computing techniques are based on an assumption that the representation of inputs and outputs is still in 2's complement format. \\




%Signed magnitude multiplication is to compute the product of magnitudes as in unsigned multiplication and then determine the product's sign by XORing the signs of the operands \ref{ref:sign-mag-Vassiliadis}. The position weights are changed only on the sign bits, and the others still rely on binary encoding system. \\

%As to the optimization of MAC units, recent explorations are conducted on the whole MAC operation.\\
%Traditional MAC unit consists of three sub-operations: Multiplication of two input values to produce partial products; First adder to compress these partial products to one or two final partial products; Second adder to accumulate the compressed partial products with the input partial sum. An proposed IMAC method is to integrate the accumulation directly into the multiplier’s partial product generation step to save both time and resources %\ref{ref:IMAC-2024}. 
%A high-performance MAC unit is designed recently by integrating a binary carry-select adder (HSBCSA) with a counter-based modular Wallace tree multiplier (CMWTM) \ref{ref:Ponraj-2023}. 
%Bit-level operation-based method is to design an efficient MAC unit by leveraging bit-level operations to optimize vector multiplications to improve computation speed and power efficiency \ref{ref:Y-bit-MAC-2023}.\\


% \spe\spb

{

\small

\begin{enumerate}[label={[}\arabic{*}{]}, resume]
    \setcounter{enumi}{3}
    \item\label{ref:D-log-2016} D. Miyashita, et al., ``Convolutional Neural Networks Using Logarithmic Data Representation,'' \textit{arXiv}, 2016.
    \item\label{ref:M-RNS-2020} M. Valueva, et al., ``Application of the Residue Number System to Reduce Hardware Costs of the Convolutional Neural Network Implementation,'' \textit{Mathematics and Computers in Simulation}, vol. 177, pp. 232–243, 2020.
    \item\label{ref:Fibonacci} W. A. Simon, et al., ``Exact Neural Networks from Inexact Multipliers via Fibonacci Weight Encoding,'' in \textit{ACM/IEEE Design Automation Conference (DAC)}, 2021.
    \item\label{ref:Booth} A. D. Booth, ``A Signed Binary Multiplication Technique,'' \textit{Quarterly Journal of Mechanics and Applied Mathematics}, vol. 4, no. 1, pp. 236–240, 1951. 
    \item\label{ref:Wallace} C. S. Wallace, ``A Suggestion for a Fast Multiplier,'' in \textit{IEEE Transactions on Electronic Computers}, 1964.
    \item\label{ref:Dadda} L. Dadda, ``Some Schemes for Parallel Multipliers,'' in \textit{IEEE Computer Society Press}, 1990.
    \item\label{ref:OMBSSM} S. Vassiliadis, et al., ``A General Proof for Overlapped Multiple-Bit Scanning Multiplications,'' \textit{IEEE Transactions on Computers (TC)}, vol. 38, no. 2, pp. 172–183, 1989.
    \item\label{ref:IMAC-2024} D. N. Devi, et al., ``Integrated MAC-based Systolic Arrays: Design and Performance Evaluation,'' in \textit{Proceedings of the Great Lakes Symposium on VLSI}, 2024.
    \item\label{ref:Ponraj-2023} J. Ponraj, et al., ``High-Performance Multiply-Accumulate Unit by Integrating Binary Carry Select Adder and Counter-Based Modular Wallace Tree Multiplier for Embedding System,'' \textit{Integration}, vol. 93, pp. 102055, 2023.
    % \item\label{ref:sign-mag-Vassiliadis} S. Vassiliadis, et al., ``Hard-Wired Multipliers with Encoded Partial Products,'' \textit{IEEE Transactions on Computers (TC)}, vol. 40, no. 11, pp. 1181-1197, 1991.
    % \item\label{ref:V-IMPACT-2011} V. Gupta, et al., ``IMPACT: IMPrecise Adders for Low-Power Approximate Computing,'' in \textit{IEEE/ACM International Symposium on Low Power Electronics and Design}, 2011.
    % \item\label{ref:J-Approximate-2013} J. Han, et al., ``Approximate Computing: An Emerging Paradigm for Energy-Efficient Design,'' in \textit{IEEE European Test Symposium (ETS)}, 2013.
    % \item\label{ref:Y-Energy-2014} Y. Kim,  et al., ``Energy Efficient Approximate Arithmetic for Error Resilient Neuromorphic Computing,'' \textit{IEEE Transactions on Very Large Scale Integration (VLSI) Systems}, vol. 23, no. 11, pp. 2733-2737, 2014.
    % \item\label{ref:EvoApprox8b-} V. Mrazek, et al., ``EvoApprox8b:  Library of Approximate Adders and Multipliers for Circuit Design and Benchmarking of Approximation Methods," in \textit{Design, Automation \& Test in Europe Conference \& Exhibition (DATE)}, 2017.
    % \item\label{ref:Y-bit-MAC-2023} Y. Feng, et al., ``Bit-Level Operation-Based MAC Unit for Vector Multiplications,'' in \textit{Science and Information Conference}, Springer Nature, 2023.
    \item\label{ref:G-Thermal-2022} G. Zervakis, et al., ``Thermal-Aware Design for Approximate DNN Accelerators,'' \textit{IEEE Transactions on Computers}, vol. 71, no.10, pp. 2687-2697, 2022.
    \item\label{ref:P-Learning-2022} P. Jain, et al., ``Learning to Design Accurate Deep Learning Accelerators with Inaccurate Multipliers,'' in \textit{Design, Automation \& Test in Europe Conference \& Exhibition (DATE)}, 2022.
    \item\label{ref:T-Toward-2024} T. Yu, et al., ``Toward Efficient Retraining: A Large-Scale Approximate Neural Network Framework With Cross-Layer Optimization,'' in \textit{IEEE Transactions on Very Large Scale Integration (VLSI) Systems}, vol. 32, no. 6, pp. 1004-1017, 2024.
\end{enumerate}

}

\vspace{20pt}

\spe\spb

\textbf{Reviewer: 2} \\

\textit{Comments to the Author}\\


\textit{1. The proposed work requires fine-tuning of the network after the new encoding scheme to regain some of the lost accuracy. This is sometimes impossible for some DNN accelerators where they treat the DNN model as blackbox provided by ISVs (integrated software vendors). It becomes difficult and sometimes impossible to do the finetuning and the only quantization you can do is PTQ. Towards that end, it would be good to see what is the accuracy impact of the encoding scheme without fine-tuning the network.}\\

\vskip 5pt

%Thanks for your concern. Actually, 
In fact 
the accuracy before fine-tuning has been reported in \figname~\ref{fig_retrain_process}, where the result at the 0-th epoch indicates the inference accuracy without fine-tuning. 
To make it clearer, 
we list the inference accuracy before, during and after fine-tuning in Table \ref{tab:finetune-resnet-acc}. As shown in this table, 
without fine-tuning, 
the inference accuracy for simple tasks, e.g., ResNet18 (Cifar-10) and ResNet20 (Cifar-100)), are still comparable compared with the accuracy with 32-bit floating-point number, while the inference accruacy for ResNet50 (ImageNet), is only 1.38\%, due to  the higher task complexity and the larger number of convolution layers. % in ResNet-50, approximation errors are accumulated to lower the accuracy. 
With fine-tuning, the accuracy for the three tasks are enhanced. Particularly for ResNet50 (ImageNet), the accuracy is recovered from 1.38\% to 74.99\% after just one epoch. 
We speed up the fine-tuning on ImageNet by randomly sampling 1\% images for each category in original training dataset during every epoch.\\
%One trick to speed-up the fine-tuning on ImageNet is to randomly sample 1\% images for each category in original training dataset during every epoch, while the inference is done on whole testing dataset.\\

{

\centering
\footnotesize
\caption{Inference accuracy before, during and after fine-tuning.}
\begin{tabular}{cccc}
\toprule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Epochs\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet18 \\(Cifar-10)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet20 \\(Cifar-100)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet50 \\(ImageNet)\end{tabular}}
\\ \midrule
w/o fine-tune     & 91.54\% & 67.23\% &  1.38\%  \\\midrule
1     & 92.51\% & 67.83\% & 74.99\%  \\
5     & 93.06\% & 68.62\% & 75.09\%  \\
10    & 92.97\% & 68.66\% & 75.45\%  \\
15    & 93.05\% & 68.83\% & 75.59\%  \\
20    & 93.05\% & 68.68\% & 75.50\%  \\
25    & 93.08\% & 68.96\% & 75.76\%  \\\midrule
32-bit FP & 93.07\% & 68.82\% & 76.15\%  \\
\bottomrule
\end{tabular}
\label{tab:finetune-resnet-acc}

}

\vskip 35pt

\textit{2. Also since the new encoding is not transparent and has accuracy impact, the authors need to try out a wide variety of DNN benchmarks across CV, NLP, LLM, VLM, Stable Diffusion, etc. The authors have tried only on ResNet which does not show whether this methodology is actually applicable to other networks. This seems to be a very small subset of possible applications.}\\

\vskip 5pt

Thanks for the suggestion. %We indeed only implement the new encoding on ResNet. 
To demonstrate the effectiveness of the proposed encoding on different types of neural networks, we  implemented MobileNetV2 \ref{ref:MobileNetV2} and EfficientNet-B0 \ref{ref:EfficientNet} with the proposed encoding. The pretrained models for MobileNetV2 (Cifar-10), MobileNetV2 (Cifar-100) and EfficientNet-B0 (ImageNet) are obtained from GitHub \ref{ref:Cifar10-models}--\ref{ref:Cifar100-models} and Torchvision \ref{ref:ImageNet-models}. 
%The new encoding is embedded 
With the new encoding, 
such neural networks are fine-tuned on an NVIDIA A100 80 GB with 10 epochs due to runtime. 
The learning rates for MobileNetV2 (Cifar-10), MobileNetV2 (Cifar-100) and EfficientNet-B0 (ImageNet) were set to 1e-4, 1e-3 and 1e-5, respectively. 
To speed up the fine-tuning of EfficientNet-B0 (ImageNet), we  randomly sampled 1\% training images in each fine-tuning epoch. For comparison, neural networks with 8-bit uniform quantization and 8-bit exact multipliers are also fine-tuned with  10 epoches. The accuracy before, during and after fine-tuning are reported in Table \ref{tab:finetune-mobilenet-efficientnet-acc} and \ref{tab:mobilenet-efficientnet-Acc}. \\

\spe\spb

According to Table \ref{tab:finetune-mobilenet-efficientnet-acc}, the accuracy without fine-tuning for MobileNetV2 (Cifar-10), MobileNetV2 (Cifar-100) and EfficientNet-B0 (ImageNet) are quite low due 
to the large number of layers.
%. An explanation might be the large number of layers in MobileNetv2 and EfficientNet-B0 accumulates the approximate errors, leading to much lower accuracies. Specifically, MobileNetv2 has 52 convolution layers. EfficientNet-B0 is deeper and has 81 convolution layers. 
However, fine-tuning can enhance the accuracy significantly. 
%For MobileNetV2 (Cifar-10) and MobileNetV2 (Cifar-100), accuracy can be recovered similar to that with 32FP configuration after just one epoch. 
For EfficientNet-B0 (ImageNet), the accuracy is improved from 0.10\% to 63.43\% after two fine-tuning epochs. 
After fine-tuning, the proposed encoding achieves slightly better accuracy than INT8 quantization with exact 8-bit multipliers for MobileNetV2 (Cifar-10) and MobileNetV2 (Cifar-100), as shown in Table \ref{tab:mobilenet-efficientnet-Acc}. 
While for large-scale EfficientNet-B0 (ImageNet), accuracy is recovered to 68.77\% after 10 epochs fine-tuning, leading to 5.30\% accuracy loss compared with INT8 quantization with exact 8-bit multipliers. 
For such large neural networks, more epoches are required for fine tuning, which could not be finished within the given time limit of this revision. 
These results have been added in Section~IV.B.
We will continue this fine tuning further to study the accuracy effect of the proposed approach as the reviewer pointed out. \\



{

\centering
\footnotesize
\caption{Inference accuracy before, during and after fine-tuning.}
\begin{tabular}{cccc}
\toprule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Epochs\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}MobileNetV2 \\(Cifar-10)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}MobileNetV2 \\(Cifar-100)\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}EfficientNet-B0 \\(ImageNet)\end{tabular}}
\\ \midrule
w/o fine-tune & 17.17\% &  9.21\% &   0.10\%  \\\midrule
      1       & 93.36\% & 70.64\% &   0.11\%  \\
      2       & 93.36\% & 70.64\% &   0.11\%  \\
      3       & 93.36\% & 70.64\% &  63.43\%  \\
      5       & 93.60\% & 70.76\% &  67.17\%  \\
      10      & 93.74\% & 71.23\% &  68.77\%  \\\midrule
      % 15      & 93.67\% & 70.53\% &       \%  \\
      % 20      & 93.66\% & 70.70\% &       \%  \\
      % 25      & 93.74\% & 71.23\% &       \%  \\\midrule
      32 FP   & 93.91\% & 71.17\% &  77.69\%  \\
\bottomrule
\end{tabular}
\label{tab:finetune-mobilenet-efficientnet-acc}

}

\vskip 5pt

{

\centering
\footnotesize
\caption{Inference accuracy comparison with 8-bit quantization.}
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{Model-Dataset} & \multirow{2}{*}{32-FP} & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}8-bit Uniform Quantization\end{tabular}} \\  \cmidrule{3-5}
                          &         &  Orig.   & Prop.      & Acc. drop          \\  \midrule
    MobileNetV2-Cifar-10  & 93.91\% &  93.70\% &   93.74\%  &  -0.04\%           \\ 
    MobileNetV2-Cifar-100 & 71.17\% &  70.72\% &   71.23\%  &  -0.51\%           \\ 
EfficientNet-B0-ImageNet  & 77.69\% &  74.07\% &   68.77\%  &  ~5.30\%           \\ 
\bottomrule
\end{tabular}
\label{tab:mobilenet-efficientnet-Acc}

}



\vskip 10pt

{

\small

\begin{enumerate}[label={[}\arabic{*}{]}, resume]
    \setcounter{enumi}{15} % 将序号起始值设为4
    \item\label{ref:MobileNetV2} M. Sandler, et al., ``MobileNetV2: Inverted Residuals and Linear Bottlenecks,'' in \textit{IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 2018.
    \item\label{ref:EfficientNet} M. Tan, et al., ``EfficientNet: Rethinking Model Scaling for Convolutional Neural Networks,'' in \textit{International Conference on Machine Learning (ICML)}, 2019.
    \item\label{ref:Cifar10-models} ``Cifar10 models,'' \url{https://github.com/huyvnphan/PyTorch_CIFAR10}.
    \item\label{ref:Cifar100-models} ``Cifar100 models,'' \url{https://github.com/weiaicunzai/pytorch-cifar100}.
    \item\label{ref:ImageNet-models} ``ImageNet models,'' \url{https://pytorch.org/vision/stable/models.html}.
\end{enumerate}

}

\vskip 20pt



\textit{3. There are existing works that have tried to do signed magnitude multiplication instead of 2's complement multiplication to reduce the switching the circuit complexity. The authors should compare their work with this approach.}\\

\vskip 5pt

%Thanks for your suggestions. ``Signed magnitude multiplication'' is a technique in digital systems where the most significant bit (MSB) is used to represent the sign (positive or negative), and the remaining bits represent the magnitude of the number. For example, decimal values in 2's complement and signed magnitude format are compared in Table \ref{tab:sig-mag-format}. 


%and the timing diagram is shown in \figname~\ref{fig:waveform-sign-mag-MAC}.\\



%{

%\centering
%\footnotesize
%\caption{Examples of decimal values in 2's complement and signed magnitude format.}
%\begin{tabular}{ccc}
%\toprule
%  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}decimal value\end{tabular}}
%& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}2's complement format\end{tabular}}
%& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}signed magnitude format\end{tabular}}
%\\ \midrule
%-4 & 100 & -        \\
%-3 & 101 & 111      \\
%-2 & 110 & 110      \\
%-1 & 111 & 101      \\
%0  & 000 & 000, 100 \\
%1  & 001 & 001      \\
%2  & 010 & 010      \\
%3  & 011 & 011      \\
%\bottomrule
%\end{tabular}
%\label{tab:sig-mag-format}

%}



To compare the area and power consumption of systolic arrays where MAC units are implemented based on 2's complement, signed magnitude and the propsoed encoding, 
we implemented MAC units based on signed magnitude format according to the  online simulation link ``\url{http://hdlbits.01xz.net/wiki/Iverilog?load=px3nzv}''. 
The comparison results are shown in 
%Area and power of 64$\times$64 MAC arrays based on 2's complement, signed magnitude and our encoding formats are compared in 
Table \ref{tab:power-area-sig-mag-MAC}. 
According to this table, 
the systolic array based on signed magnitude format achieves lower power, but larger area than the one with 2's complement. The proposed encoding can achieve the smallest 
area overhead and power consumption. This comparison has been added in Section~\ref{Hardware Comparison with Signed Magnitude Systolic Arrays}. \\

%{

%\centerline{\includegraphics[width=0.8\linewidth]{./Figs/waveform-sign-mag.pdf}}
%\captionof{figure}{The timing diagram of a MAC unit based on signed magnitude multiplication and accumulation.}
%\label{fig:waveform-sign-mag-MAC}

%}

\vskip 5pt

{

\centering
\footnotesize
\begin{minipage}{1\textwidth}  % 设置minipage的宽度为表格宽度
\centering
\caption{Power and area comparison between MAC units based on 2's complement, signed magnitude  and the proposed enconding.}
\begin{tabular}{cccccccccc}
\toprule
  \multirow{2}{*}{Architecture} &
& \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Multiplier\end{tabular}}  &
& \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Accumulator\end{tabular}} &
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Area (mm$^2$)\\64$\times$64\end{tabular}}
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Power (W)\\64$\times$64\end{tabular}}
\\ \cmidrule{3-4}\cmidrule{6-7}
         & & input       & output       & & input        & output        & &      &      \\ \midrule
systolic & & 2's comp.   & 2's comp.    & & 2's comp.    & 2's comp.     & & 0.76 & 3.82 \\
systolic & & signed mag. & signed mag.  & & signed mag.  & signed mag.   & & 0.88 & 3.22 \\
proposed & & 2's comp.   & ours         & & ours         & 2's comp.     & & 0.58 & 2.17 \\
\bottomrule
\end{tabular}
\label{tab:power-area-sig-mag-MAC}
\end{minipage}

}

\spe\spb

\vskip 30pt


\textit{4. Given fine-tuning is involved, a better option will be to go to heavily quantized networks with INT2/INT4/INT6 activations weights. They all may result in a better power-accuracy tradeoff than encoding net. A comparison of the same is missing in the paper.}\\

\vskip 5pt

Thanks for your suggestion. Accuracy of heavily quantized networks are reported in Table \ref{tab:int-nn-acc-power-area}. We also implemented the 
 64$\times$64 MAC array with the corresponding quantized MAC units and evaluated the resulting area and power, as shown in the following table. To extensively evaluate the quantization configurations, we swept all combinations of INT2/INT4/INT6/INT8 activations and weights, and fine-tuning technique was also applied to enhance the inference accuracy. 
 %Assume [INT$n$/INT$n$] represents the quantization scheme for $n$-bit activations and $n$-bit weights. 
 For ResNet 18 on Cifar-10, accuracy can be well maintained on [INT6/INT4], [INT6/INT6], [INT6/INT8], [INT8/INT4], [INT8/INT6], and [INT8/INT8]. Power and area of [INT6/INT4] and [INT8/INT4] are indeed smaller than our proposed method. But for ResNet 20 on Cifar-100, accuracy can only well maintained on [INT8/INT6] and [INT8/INT8], and the power and area are both larger than ours. For ResNet 50 on ImageNet, accuracy can only be maintained on [INT8/INT8] and the implementation of the corresponding systolic arrays incurs the largest power and area. Generally, the proposed method can balance accuracy, area overhead and power consumption for deep neural networks. This comparison has been added in Section~\ref{Hardware and Accuracy Comparison with Integer Quantization}.\\

{

\centering
\footnotesize
\caption{Accuracy comparison of neural networks on various quantization bit-widths for weights and activations after fine-tuning, as well as the corresponding power and area with the quantization configuration.}
\begin{tabular}{cccccccc}
\toprule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Architecture\end{tabular}}  
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Activations\end{tabular}}  
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Weights\end{tabular}} 
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet18 \\(Cifar-10)\\FP32: 93.07\%\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet20 \\(Cifar-100)\\FP32: 68.82\%\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ResNet50 \\(ImageNet)\\FP32: 76.15\%\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Area (mm$^2$)\\64$\times$64\end{tabular}}
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Power (W)\\64$\times$64\end{tabular}}
\\ \midrule
Systolic & INT2 & INT2 & 10.00\% &  1.00\%  &  0.10\% & 0.1705  & 0.8036  \\
Systolic & INT2 & INT4 & 65.65\% &  6.21\%  &  0.12\% & 0.2297  & 1.0617  \\
Systolic & INT2 & INT6 & 66.34\% & 12.82\%  &  0.15\% & 0.2581  & 1.2390  \\
Systolic & INT2 & INT8 & 66.77\% & 14.95\%  &  0.13\% & 0.3032  & 1.4635  \\ \midrule
Systolic & INT4 & INT2 & 86.83\% &  1.00\%  &  0.10\% & 0.2293  & 1.0633  \\
Systolic & INT4 & INT4 & 90.88\% & 54.70\%  & 44.29\% & 0.3096  & 1.3119  \\
Systolic & INT4 & INT6 & 90.70\% & 57.32\%  & 51.66\% & 0.3721  & 1.8248  \\
Systolic & INT4 & INT8 & 91.30\% & 60.13\%  & 52.06\% & 0.4878  & 2.5895  \\ \midrule
Systolic & INT6 & INT2 & 90.66\% &  5.10\%  &  0.10\% & 0.2579  & 1.1665  \\
Systolic & INT6 & INT4 & 92.64\% & 58.99\%  & 46.97\% & 0.3721  & 1.5888  \\
Systolic & INT6 & INT6 & 93.08\% & 65.52\%  & 66.70\% & 0.4989  & 2.5498  \\
Systolic & INT6 & INT8 & 92.91\% & 65.85\%  & 71.75\% & 0.6106  & 2.9696  \\ \midrule
Systolic & INT8 & INT2 & 90.36\% &  1.00\%  &  0.10\% & 0.3030  & 1.3836  \\
Systolic & INT8 & INT4 & 92.86\% & 60.95\%  & 47.20\% & 0.4504  & 1.9145  \\
Systolic & INT8 & INT6 & 92.97\% & 67.95\%  & 71.92\% & 0.5957  & 2.4560  \\
Systolic & INT8 & INT8 & 93.13\% & 68.40\%  & 75.64\% & 0.7560  & 3.8003  \\ \midrule
Proposed & INT8 & INT8 & 93.14\% & 68.32\%  & 75.46\% & 0.5800  & 2.1700  \\ % \midrule
% Systolic & FP32 & FP32 & 93.07\% & 68.82\%  & 76.15\% & -       & -      \\
\bottomrule
\end{tabular}
\label{tab:int-nn-acc-power-area}

}



\vskip 20pt



\renewcommand{\thetable}{\arabic{table}}
\setcounter{table}{0}

\spe
\reviewe

==> tb3.tex <==


\begin{table*}[htbp]
\setlength{\tabcolsep}{4.8pt}%2.5pt
\renewcommand{\arraystretch}{1.2}
\centering
\caption{Software and hardware scheme configuration and notation.}
\small
\begin{tabular}{cccccccccc}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Platform\end{tabular}}
 &
   \multicolumn{5}{c}{Software Scheme} & 
   &
  \multicolumn{3}{c}{Hardware Scheme} \\ \cmidrule{2-6} \cmidrule{8-10}
 &
  Quantization &
  \begin{tabular}[c]{@{}c@{}}Layers\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Levels\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Proposed Encoding\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Notation\end{tabular} &
   &
  \begin{tabular}[c]{@{}c@{}}Decoder\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Systolic Array\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Notation\end{tabular} \\
  \midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}General-Purpose\end{tabular}} &
    \begin{tabular}[c]{@{}c@{}}8-bit Uniform\end{tabular}     &  all    &  same      &  no  &  8UQ-Orig.-all   &   &  no  &  original &  G-HW-Orig. \\
 &  \begin{tabular}[c]{@{}c@{}}8-bit Uniform\end{tabular}     &  all    &  same      &  yes &  8UQ-Prop.-all   &   &  no  &  proposed &  G-HW-Prop. \\
 &  \begin{tabular}[c]{@{}c@{}}4-bit Non-Uniform\end{tabular} &  all    &  different &  no  &  4NUQ-Orig.-all  &   &  yes &  original &  G-HW-Orig.+D \\
 &  \begin{tabular}[c]{@{}c@{}}4-bit Non-Uniform\end{tabular} &  all    &  different &  yes &  4NUQ-Prop.-all  &   &  yes &  proposed &  G-HW-Prop.+D \\
 &  \begin{tabular}[c]{@{}c@{}}4-bit Non-Uniform\end{tabular} &  middle &  different &  no  &  4NUQ-Orig.-mid. &   &  yes &  original &  G-HW-Orig.+D \\
 &  \begin{tabular}[c]{@{}c@{}}4-bit Non-Uniform\end{tabular} &  middle &  different &  yes &  4NUQ-Prop.-mid. &   &  yes &  proposed &  G-HW-Prop.+D \\
  \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Specific-Purpose\end{tabular}} &
    \begin{tabular}[c]{@{}c@{}}4-bit Non-Uniform\end{tabular} &  all    &  same      &  no  &  4NUQ-Orig.      &   &  yes &  original &  G-HW-Orig.+D \\
 &  \begin{tabular}[c]{@{}c@{}}4-bit Non-Uniform\end{tabular} &  all    &  same      &  yes &  4NUQ-Prop.      &   &  no  &  proposed &  S-HW-Prop. \\
  \bottomrule
\end{tabular}
\end{table*}



